Injecting Numerical Reasoning Skills into Knowledge Base Question Answering Models

Embedding-based methods are popular for Knowledge Base Question Answering (KBQA), but few current models have numerical reasoning skills and thus struggle to answer ordinal constrained questions. This paper proposes a new embedding-based KBQA framework which particularly takes numerical reasoning into account. We present NumericalTransformer on top of NSM, a state-of-the-art embedding-based KBQA model, to create NT-NSM. To enable better training, we propose two pre-training tasks with explicit numerical-oriented loss functions on two generated training datasets and a template-based data augmentation method for enriching ordinal constrained QA dataset. Extensive experiments on KBQA benchmarks demonstrate that with the help of our training algorithm, NT-NSM is empowered with numerical reasoning skills and substantially outperforms the baselines in answering ordinal constrained questions.

==> pretraining_1.tex <==
 \begin{figure*}[t]
	\centering
	\includegraphics[width=0.85\textwidth]{numericaldata_1}
	\caption{\label{fig:numericaldata} Two kinds of automatically generated datasets for pre-training \model.}
\end{figure*}



\section{Pre-training and Data Augmentation}
\label{sec:training}
\subsection{Pre-training Tasks}
\label{sec:pretraining}
%The \swmodel is trained by the end-to-end KBQA task. 
Although the \smodel in \swmodel allows the rich interactions between the question words and the numbers, the number embeddings are learned implicitly without the explicit annotation of the two numerical properties in the standard KBQA training data. To enhance the number embeddings, we propose two pre-training tasks according to the two numerical properties by generating two kinds of training data $\{( q, r, \mathcal{V}_r, v_q)\}$
%As shown in Figure~\ref{fig:numericaldata}, the input of \smodel in pre-training is comprised of the ordinal determiner/the question $q$, the relation $r$ and the numbers $\mathcal{V}_r$ which include the correct answer number $v_q$. 
and defining two objective functions on top of the training data. The \smodel is only pre-trained once on the generated training data and then it can be adapted to all KBQA datasets and basic reasoning models.



% We verify the drawback by performing an explicit number prediction task.
% Specifically, we test \swmodel on questions from CWQ~\citep{talmor-berant-2018-web}'s ordinal constrained QA test set to obtain number embeddings. We determine the correct number that satisfies the question following the below QGND generation process, predict it based on its number embedding and obtain 42.3 \% of Hits@1. We observe that Hits@1 of QA task is 55.5\% on the instances that the true number can be correctly predicted, and only 13.3\% on the wrongly predicted instances, which demonstrates the crucial effect of accurate number prediction.
% We conjecture that number embedding learning could benefit from explicit supervision and propose two pre-training tasks based on two kinds of generated training data for pre-training the parameters $\Theta$ of \model. 

\vpara{Question-irrelevant Numerical Dataset (QIND).}
Considering the difficulty of creating a textual question, we generate a question-irrelevant dataset on a large scale.
Specifically, we randomly extract a set of numerical relations from $\mathcal{G}$ and sample $N$  numbers associated with each relation $r$ into $\mathcal{V}_r$. Then we choose an ordinal determiner $q$ and annotate the number in $\mathcal{V}_r$ satisfying $q$ as the correct answer $v_q$. The tuple $(q,r,\mathcal{V}_r,v_q)$ composes a training instance. The ordinal determiners include ``largest'', ``fewest'', ``biggest'', and ``smallest'' for size-based numerical relations and ``earliest'', ``latest'', ``most recent'', ``first'', and ``last'' for time-based numerical relations. 
Figure~\ref{fig:numericaldata} illustrates a generated instance, where ``12 20 48 100'' are the numbers associated with the relation ``tv.program.num\_of\_episodes''. ``100'' can be automatically annotated as the correct answer guided by the ordinal determiner ``largest''. 

\vpara{Question-guided Numerical Dataset (QGND).}
We create a second question-guided dataset to enhance the connection with authentic data. Specifically, we retrieve ordinal constrained QA pairs from CWQ's training dataset.\footnote{Other datasets indicating the relationship between ordinal determiners and numbers can also be chosen for creating QGND.}
For each QA pair $(q,a_q)$, we select the relevant $r$ that can derive the answer, and include the number $v$ satisfying $(a_q, r, v) \in \mathcal{G}$ as the correct number $v_q$ into $\mathcal{V}_r$. Then we add several other numbers associated with $r$ into $\mathcal{V}_r$. Figure~\ref{fig:numericaldata} illustrates an instance.

% where ``Of the films in which Kim Richards acted, which was released latest?" is a chosen question and ``2009.08.04" is the correct number.
%, as it is associated with the relevant relation ``film.film.release\_date" and the answer ``Race to Witch Mountain". 


\vpara{Pre-training Objectives.}
% Suppose $\{(q,r,\mathcal{V}_r, a_q)\}$ denotes the training data which combines both QIND and QGND. 
We propose a number-aware triplet loss (NTL) and a number prediction loss (NPL) and optimize them on QIND first and then on QGND.
NTL aims to preserve the relative magnitude of numbers. For each instance $( q, r, \mathcal{V}_r, v_q )$, we randomly sample three numbers from $\mathcal{V}_r$ and allow the small number $v_s$ to be closer to the median one $v_m$ than the big one $v_b$. In another word, ``$v_s \prec v_m\prec v_b$''  should be satisfied.
% to reflect the relative distance between numbers rather than the absolute magnitude. 
The loss function is:
% \vspace{-0.005cm}   
\beq{
\small
\label{eq:numbertripletloss}
\ell^1 =\sum_{(v_s,v_m,v_b) \in \mathcal{T}}{\rm max}(0,\epsilon+ g(\textbf{v}_s,\textbf{v}_m)-g(\textbf{v}_s,\textbf{v}_b)),
}
\normalsize

\noindent where $g$ is the cosine similarity between two numbers, $\textbf{v}$ is the output number embedding of \model, $\mathcal{T}$ is the set of the sampled triplets, and $\epsilon$ is a margin separating $(v_s,v_m)$ and $(v_s,v_b)$.

NPL captures the ordinal relationship.
% between the ordinal determiner and the numbers. 
For example, we aim to make the embedding of 1 in ``$1\prec2\prec3$'' 
 closer to the ordinal determiner ``smallest'' than 2 and 3. 
For a generated instance, we predict the probability of $v_i$ being the answer as:
% \vspace{-0.005cm}  
\beq{
\small
\label{eq:numberpredictionloss}
p(v_i \vert q, r,\mathcal{V}_r )= \frac{\exp \sigma( \textbf{W}_{\rm pretrain}^{\top} (\textbf{v}_i))}{\sum_{v_j \in \mathcal{V}_r} \exp \sigma( \textbf{W}_{\rm pretrain}^{\top}(\textbf{v}_j))},
}
\normalsize

\noindent where $\textbf{W}_{\rm pretrain}$ with  $\Theta$ are trained by a cross-entropy loss. 
\begin{figure}[t]
	\centering
	\includegraphics[width=0.44\textwidth]{Figures/QApairs}
	\caption{\label{fig:qapairs} A generated ordinal constrained QA pair.}
\end{figure}
We train NTL and NPL together.

\subsection{Data Augmentation}
\label{sec:QA_pairs}
\vpara{Issue of Insufficient Training.} The ordinal constrained QA pairs are usually much fewer than the normal QA pairs on the existing KBQA benchmarks, which may cause the insufficient training of the proposed model.
To verify our hypothesis, we conduct a quick experiment on the CWQ dataset. 
% We first train the model in Eq.\ref{eq:typeprediction} on the CWQ training dataset without any pre-training and find that its test performance is 28.9\% Hits@1 on the subset of ordinal constrained QA pairs. Then 
We reduce the ordinal constrained QA pairs by half in the original training dataset and re-train the model in Eq.\ref{eq:typeprediction}, which results in a drastic drop (-8\% Hits@1) of the ordinal constrained QA performance. 
To overcome this issue, we propose a template-based data augmentation method for increasing the ordinal constrained supervision signals and train the model on the union of the standard training data and the augmented data. 
% , which includes generating augmented data and training the model on the union of the standard training data and the augmented data. 

% which also increases the difficulty of ordinal constrained KBQA. 
% For example, on CWQ's ordinal constrained QA test data, \swmodel with pre-training can obtain 42.1\% Hits@1, which drops to 37.1\% when the ordinal constrained training instances are reduced by half. 

\vpara{Generating Ordinal Constrained QA Pairs.} %Our key idea is to automatically generate some pseudo ordinal constrained QA pairs by using a template-based method. 
We first randomly select a numerical relation $r$ from $\mathcal{G}$ and sample the entities and the corresponding numerical values satisfying $\{(e,r,v)\in \mathcal{G}\}$. Then starting from those entities $\{e\}$ as tails, we trace back to their first-order neighbors $\{(e_h,r_h)\}$. Finally, we choose the entities that share the same $(e_h,r_h)$ as the candidate entities $\mathcal{C}$. The textual question is constructed according to the template ``What is the [$r_h$] of [$e_h$] that has the [ordinal determiner] [$r$] ?''. The answer is selected from $\mathcal{C}$ with the numerical value that satisfies the instantiated ordinal determiner. Figure~\ref{fig:qapairs} shows a generated example, where ``area'' is the selected numerical relation. Based on it, ``Shenzhen'', ``Beijing'', and ``Shanghai'' and their corresponding areas are sampled. From them, we trace back to the common entity ``China'' and the relation ``city''. Finally, ``Beijing'' with the ``largest'' (the instantiated ordinal determiner) area ``6,490 mi$^2$'' is annotated as the answer.

\vpara{Overall Training Algorithm.} 
Algorithm~\ref{algo:training} presents the entire training process, where 
$\Phi$ of NSM (basic reasoning), $\Theta$ of \smodel (numerical reasoning), and $\Psi$ of the comprehensive reasoning module are parameters to be optimized. $\Theta$ of \smodel is only updated in pre-training and is frozen in numerical reasoning, which significantly improve the inference efficiency. More specifically, after pre-training $\Phi$ and $\Theta$, $\Phi$ excluding $\Theta$ is fine-tuned with $\Psi$, because the pre-trained $\Theta$ is good enough for capturing numerical properties, while fine-tuning $\Phi$ after being injected the number embeddings is for better answer selection. 

% \begin{algorithm}[t]
%     \footnotesize{
%      \caption{ Training by Pre-training and DA\label{algo:training}}
%     \KwIn{The KB, QIND, QGND, real and pseudo QA data.}
%     \KwOut{Learned parameters $\Phi$, $\Theta$, and $\Psi$.}
%     \STATE Initialize $\{\textbf{e}, \textbf{r}, \textbf{v}, \textbf{q}\}$ by RoBERTa;\\
%     Pre-train $\Phi$ by Cross-entropy of Eq.~\ref{eq:basicpredict} on the real QA data;\\
%     Pre-train $\Theta$ by Eq.~\ref{eq:numbertripletloss} and Eq.~\ref{eq:numberpredictionloss} on QIND and QGND;\\
%     Retrieve $(\mathcal{G}_q,\mathcal{R}_q,\mathcal{V}_q)$ for each $q$;\\
%     Apply NSM to update $\{\textbf{e}\}$ by Eq.~\ref{eq:basicembedding};\\
%     Apply \smodel to update $\{\textbf{v}\}$ by Eq.~\ref{eq:transformerinput}-\ref{eq:mask};\\
%     Fuse $\{\textbf{v}\}$ into the pruned $\{\textbf{e}\}$ by Eq.~\ref{eq:numberplugin}-\ref{eq:finalembedding};\\
%     Train $\Phi$ and $\Psi$ by Cross-entropy of Eq.~\ref{eq:typeprediction} on real and pseudo QA data.
%     }
%  \end{algorithm}




